Incentivising Demand Side Response through Discount Scheduling using Hybrid Quantum Optimization

Demand Side Response (DSR) is a strategy that enables consumers to actively participate in managing electricity demand. It aims to alleviate strain on the grid during high demand and promote a more balanced and efficient use of (renewable) electricity resources. We implement DSR through discount scheduling, which involves offering discrete price incentives to consumers to adjust their electricity consumption patterns to times when their local energy mix consists of more renewable energy. Since we tailor the discounts to individual customers' consumption, the Discount Scheduling Problem (DSP) becomes a large combinatorial optimization task. Consequently, we adopt a hybrid quantum computing approach, using D-Wave's Leap Hybrid Cloud. We benchmark Leap against Gurobi, a classical Mixed Integer optimizer in terms of solution quality at fixed runtime and fairness in terms of discount allocation. Furthermore, we propose a large-scale decomposition algorithm/heuristic for the DSP, applied with either quantum or classical computers running the subroutines, which significantly reduces the problem size while maintaining solution quality. Using synthetic data generated from real-world data, we observe that the classical decomposition method obtains the best overall \newp{solution quality for problem sizes up to 3200 consumers, however, the hybrid quantum approach provides more evenly distributed discounts across consumers.

==> sections/04_data_generation.tex <==
\section{Data Generation}\label{sec:data_generation}

Brief overview of the synthetic data generation library. (E.ON, Giorgio)



==> sections/data_table_full.tex <==
    \begin{tabular}{llrrrrr}
    $N_C$ & Solver& Rel. Cost Err. & Rel. CO$_2$ Red. Err. & Cons. Deviation Std. & Avg. Discount Changes & Avg. Rel. Savings \\ \hline
\midrule
\textbf{25  } & \textbf{Gurobi} &         0.0156 &                   0.0126 &               0.0376 &                 0.164 &            0.0369 \\
     & \textbf{Leap} &          0.221 &                     0.22 &               0.0271 &                 0.785 &             0.137 \\
     & \textbf{Leap} &          0.292 &                     0.29 &               0.0352 &                 0.764 &             0.146 \\
     & \textbf{Leap} &          0.818 &                    0.816 &               0.0399 &                 0.787 &             0.116 \\ \hline
\textbf{50  } & \textbf{Decomp-Gurobi[50]} &        0.00036 &                 0.000495 &              0.00679 &                 0.196 &            0.0505 \\
     & \textbf{Decomp-Leap[50]} &         0.0541 &                    0.535 &                0.091 &                 0.722 &              0.14 \\
     & \textbf{Decomp-Leap[50]} &         0.0574 &                    0.405 &               0.0775 &                 0.741 &             0.132 \\
     & \textbf{Decomp-Leap[50]} &         0.0605 &                    0.867 &               0.0781 &                 0.729 &             0.132 \\
     & \textbf{Gurobi} &         0.0406 &                   0.0403 &               0.0145 &                0.0724 &            0.0153 \\
     & \textbf{Leap} &          0.803 &                      0.8 &               0.0428 &                 0.797 &             0.115 \\
     & \textbf{Leap} &          0.744 &                    0.741 &               0.0458 &                 0.802 &             0.118 \\
     & \textbf{Leap} &          0.798 &                    0.795 &               0.0412 &                 0.804 &             0.119 \\ \hline
\textbf{100 } & \textbf{Decomp-Gurobi[50]} &       2.02e-05 &                 4.96e-06 &              0.00338 &                 0.299 &             0.105 \\
     & \textbf{Decomp-Leap[50]} &         0.0225 &                   0.0727 &               0.0598 &                 0.416 &              0.23 \\
     & \textbf{Decomp-Leap[50]} &         0.0147 &                   0.0142 &               0.0603 &                 0.554 &             0.196 \\
     & \textbf{Decomp-Leap[50]} &         0.0327 &                    0.134 &               0.0631 &                 0.402 &             0.227 \\
     & \textbf{Gurobi} &        0.00655 &                  0.00631 &              0.00973 &                0.0813 &            0.0169 \\
     & \textbf{Leap} &          0.141 &                    0.138 &               0.0381 &                  0.79 &             0.139 \\
     & \textbf{Leap} &         0.0756 &                   0.0738 &               0.0327 &                 0.771 &              0.14 \\
     & \textbf{Leap} &         0.0045 &                  0.00283 &               0.0272 &                  0.74 &             0.149 \\ \hline
\textbf{200 } & \textbf{Decomp-Gurobi[50]} &       0.000188 &                 0.000309 &              0.00488 &                  0.27 &             0.103 \\
     & \textbf{Decomp-Leap[50]} &        0.00908 &                  0.00453 &               0.0592 &                 0.481 &             0.214 \\
     & \textbf{Decomp-Leap[50]} &        0.00437 &                 1.78e-05 &               0.0479 &                 0.553 &             0.193 \\
     & \textbf{Decomp-Leap[50]} &        0.00423 &                 0.000131 &                0.047 &                 0.556 &             0.192 \\
     & \textbf{Gurobi} &          0.918 &                    0.911 &                0.067 &                 0.497 &             0.251 \\
     & \textbf{Leap} &         0.0869 &                    0.084 &               0.0412 &                 0.786 &             0.135 \\
     & \textbf{Leap} &        0.00406 &                  0.00181 &               0.0345 &                 0.744 &             0.144 \\
     & \textbf{Leap} &        0.00522 &                  0.00214 &               0.0371 &                 0.743 &             0.152 \\ \hline
\textbf{400 } & \textbf{Decomp-Gurobi[50]} &       0.000173 &                 1.01e-06 &              0.00924 &                 0.302 &             0.113 \\
     & \textbf{Decomp-Leap[50]} &        0.00393 &                 8.68e-06 &               0.0464 &                 0.453 &             0.238 \\
     & \textbf{Decomp-Leap[50]} &        0.00372 &                 3.64e-05 &               0.0446 &                 0.494 &             0.223 \\
     & \textbf{Decomp-Leap[50]} &        0.00299 &                 3.69e-06 &               0.0408 &                 0.481 &             0.227 \\
     & \textbf{Gurobi} &           1.02 &                     1.01 &               0.0632 &                 0.494 &             0.251 \\
     & \textbf{Leap} &        0.00651 &                  0.00385 &               0.0379 &                 0.764 &             0.138 \\
     & \textbf{Leap} &       0.000485 &                   0.0883 &               0.0386 &                 0.751 &             0.138 \\
     & \textbf{Leap} &        0.00184 &                   0.0877 &               0.0387 &                  0.75 &              0.14 \\ \hline
\textbf{800 } & \textbf{Decomp-Gurobi[50]} &       0.000177 &                 3.61e-07 &              0.00942 &                 0.293 &             0.109 \\
     & \textbf{Decomp-Leap[50]} &        0.00284 &                 1.15e-06 &                 0.04 &                 0.478 &             0.229 \\
     & \textbf{Decomp-Leap[50]} &        0.00319 &                 1.13e-07 &               0.0425 &                 0.431 &             0.246 \\
     & \textbf{Decomp-Leap[50]} &        0.00233 &                 5.85e-07 &               0.0363 &                 0.543 &             0.208 \\
     & \textbf{Gurobi} &           1.11 &                      1.1 &               0.0631 &                 0.492 &             0.253 \\
     & \textbf{Leap} &         0.0179 &                   0.0148 &               0.0428 &                 0.781 &             0.131 \\
     & \textbf{Leap} &        0.00778 &                  0.00476 &               0.0416 &                  0.77 &             0.133 \\
     & \textbf{Leap} &         0.0208 &                   0.0176 &               0.0435 &                 0.777 &             0.131 \\ \hline
\textbf{1600} & \textbf{Decomp-Gurobi[50]} &       0.000134 &                 1.65e-08 &               0.0079 &                 0.289 &             0.111 \\
     & \textbf{Decomp-Leap[50]} &         0.0027 &                 7.32e-08 &               0.0391 &                 0.492 &             0.226 \\
     & \textbf{Decomp-Leap[50]} &        0.00303 &                 3.87e-07 &               0.0415 &                 0.475 &             0.231 \\
     & \textbf{Decomp-Leap[50]} &        0.00244 &                 7.63e-08 &                0.037 &                  0.49 &             0.227 \\
     & \textbf{Gurobi} &          0.962 &                    0.956 &               0.0627 &                 0.493 &              0.25 \\
     & \textbf{Leap} &        0.00719 &                  0.00422 &               0.0391 &                 0.732 &             0.156 \\
     & \textbf{Leap} &        0.00135 &                 0.000411 &               0.0205 &                 0.737 &             0.156 \\
     & \textbf{Leap} &        0.00111 &                 3.97e-05 &               0.0219 &                  0.62 &             0.198 \\ \hline
\textbf{3200} & \textbf{Decomp-Gurobi[50]} &       0.000256 &                 1.26e-08 &               0.0117 &                 0.291 &             0.109 \\
     & \textbf{Decomp-Leap[50]} &        0.00248 &                 5.65e-08 &               0.0373 &                 0.482 &              0.23 \\
     & \textbf{Decomp-Leap[50]} &        0.00228 &                 1.87e-06 &               0.0358 &                 0.513 &             0.219 \\
     & \textbf{Decomp-Leap[50]} &        0.00244 &                 1.48e-08 &               0.0371 &                 0.499 &             0.222 \\
     & \textbf{Gurobi} &          0.999 &                    0.992 &                0.063 &                 0.492 &             0.251 \\
     & \textbf{Leap} &        0.00611 &                  0.00475 &               0.0261 &                 0.712 &             0.168 \\
     & \textbf{Leap} &        0.00752 &                  0.00518 &               0.0366 &                 0.747 &             0.137 \\
     & \textbf{Leap} &         0.0201 &                    0.017 &               0.0419 &                 0.772 &             0.124 \\
\bottomrule
    \end{tabular}

==> sections/data_table_mean.tex <==
    \begin{tabular}{llrrrrr}
    $N_C$ & Solver& Rel. Cost Err. & Rel. CO$_2$ Red. Err. & Cons. Deviation Std. & Avg. Discount Changes & Avg. Rel. Savings \\ \hline
\midrule
\textbf{25  } & \textbf{Gurobi} &         0.0156 &                   0.0126 &               0.0376 &                 0.164 &            0.0369 \\
     & \textbf{Leap} &          0.444 &                    0.442 &               0.0341 &                 0.779 &             0.133 \\  \hline
\textbf{50  } & \textbf{Decomp-Gurobi[50]} &        0.00036 &                 0.000495 &              0.00679 &                 0.196 &            0.0505 \\
     & \textbf{Decomp-Leap[50]} &         0.0574 &                    0.602 &               0.0822 &                 0.731 &             0.135 \\
     & \textbf{Gurobi} &         0.0406 &                   0.0403 &               0.0145 &                0.0724 &            0.0153 \\
     & \textbf{Leap} &          0.782 &                    0.778 &               0.0433 &                 0.801 &             0.118 \\  \hline
\textbf{100 } & \textbf{Decomp-Gurobi[50]} &       2.02e-05 &                 4.96e-06 &              0.00338 &                 0.299 &             0.105 \\
     & \textbf{Decomp-Leap[50]} &         0.0233 &                   0.0737 &               0.0611 &                 0.457 &             0.218 \\
     & \textbf{Gurobi} &        0.00655 &                  0.00631 &              0.00973 &                0.0813 &            0.0169 \\
     & \textbf{Leap} &         0.0737 &                   0.0717 &               0.0327 &                 0.767 &             0.143 \\  \hline
\textbf{200 } & \textbf{Decomp-Gurobi[50]} &       0.000188 &                 0.000309 &              0.00488 &                  0.27 &             0.103 \\
     & \textbf{Decomp-Leap[50]} &        0.00589 &                  0.00156 &               0.0514 &                  0.53 &               0.2 \\
     & \textbf{Gurobi} &          0.918 &                    0.911 &                0.067 &                 0.497 &             0.251 \\
     & \textbf{Leap} &          0.032 &                   0.0293 &               0.0376 &                 0.757 &             0.143 \\  \hline
\textbf{400 } & \textbf{Decomp-Gurobi[50]} &       0.000173 &                 1.01e-06 &              0.00924 &                 0.302 &             0.113 \\
     & \textbf{Decomp-Leap[50]} &        0.00355 &                 1.63e-05 &                0.044 &                 0.476 &             0.229 \\
     & \textbf{Gurobi} &           1.02 &                     1.01 &               0.0632 &                 0.494 &             0.251 \\
     & \textbf{Leap} &        0.00295 &                     0.06 &               0.0384 &                 0.755 &             0.139 \\  \hline
\textbf{800 } & \textbf{Decomp-Gurobi[50]} &       0.000177 &                 3.61e-07 &              0.00942 &                 0.293 &             0.109 \\
     & \textbf{Decomp-Leap[50]} &        0.00279 &                 6.14e-07 &               0.0396 &                 0.484 &             0.227 \\
     & \textbf{Gurobi} &           1.11 &                      1.1 &               0.0631 &                 0.492 &             0.253 \\
     & \textbf{Leap} &         0.0155 &                   0.0124 &               0.0426 &                 0.776 &             0.131 \\  \hline
\textbf{1600} & \textbf{Decomp-Gurobi[50]} &       0.000134 &                 1.65e-08 &               0.0079 &                 0.289 &             0.111 \\
     & \textbf{Decomp-Leap[50]} &        0.00272 &                 1.79e-07 &               0.0392 &                 0.485 &             0.228 \\
     & \textbf{Gurobi} &          0.962 &                    0.956 &               0.0627 &                 0.493 &              0.25 \\
     & \textbf{Leap} &        0.00322 &                  0.00156 &               0.0272 &                 0.696 &              0.17 \\  \hline
\textbf{3200} & \textbf{Decomp-Gurobi[50]} &       0.000256 &                 1.26e-08 &               0.0117 &                 0.291 &             0.109 \\
     & \textbf{Decomp-Leap[50]} &         0.0024 &                 6.46e-07 &               0.0367 &                 0.498 &             0.223 \\
     & \textbf{Gurobi} &          0.999 &                    0.992 &                0.063 &                 0.492 &             0.251 \\
     & \textbf{Leap} &         0.0112 &                  0.00899 &               0.0349 &                 0.744 &             0.143 \\
\bottomrule
    \end{tabular}

==> sections/qpu_evaluations/01_original.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{graphics/plots/qpu/legend.pdf}\\
    \includegraphics[width=0.24\textwidth,trim=0 15 0 0,clip]{graphics/plots/qpu/bench_rel_co2_reduction.pdf}%
    \includegraphics[width=0.24\textwidth,trim=0 15 0 0,clip]{graphics/plots/qpu/bench_rel_energy.pdf}\\
    \includegraphics[width=0.24\textwidth,trim=0 15 0 0,clip]{graphics/plots/qpu/bench_consumption_deviation.pdf}%
    \includegraphics[width=0.24\textwidth,trim=0 15 0 0,clip]{graphics/plots/qpu/bench_discount_change.pdf}\\
    \includegraphics[width=0.24\textwidth]{graphics/plots/qpu/bench_price_change.pdf}%
    \includegraphics[width=0.24\textwidth]{graphics/plots/qpu/bench_time.pdf}%
    \caption{All metrics for the small problem sizes, also considering QUBO sub-problems that can be solved using D-Wave's QPU.
    Again, we observe the cut in performance for \texttt{Gurobi} between 240 and 480 customers. Notably, the \texttt{Decomp} solvers exhibit equal per-customer metric measurements in all problem sizes. To match the runtime of the other solvers, i.e., the \texttt{Decomp-QPU}, we had to manually adjust the number of reads from the simulated annealing routine to 30. We also observe, that \texttt{Leap} outruns the set timeout here, which we do not adjust since the baseline is \texttt{Decomp-QPU}.}
    \label{fig:eval-qpu}
\end{figure}

Fig.~\ref{fig:eval-embedding-size} shows the computed embeddings for the sub-problem QUBOs with different problem sizes. It is apparent that we are very limited to small problem sizes. Since we do not want too few customers in a chunk to preserve flexibility, we settle at a reasonable middle ground of chunk size six and $12$ timesteps. We interpolate the original data to 12 timesteps and use various (multiples of 6) customer sizes to compare the performance of \texttt{Decomp-QPU} against the other solvers. For each sub-problem, we take 100 readings from the QPU. We cannot directly steer the timeout in this case. Thus, we chose to first run \texttt{Decomp-QPU} and then set the timeout of the remaining solvers to exactly that time. However, \texttt{Leap} has a minimum runtime of 5\,s, which is the reason why we only include \texttt{Leap} in the cases where the \texttt{Decomp-QPU} time is more than 5\,s, being the case from $N_c = 480$ onwards.

We again perform the analysis for different problem sizes, reaching from 60 to 1920 customers, or 720 to 23,040 integer variables. The sub-problems consist of 72 integer variables, resulting in 216 binary variables in the QUBO formulation. Fig.~\ref{fig:eval-qpu} displays the results of these experiments. Likewise to the earlier experiments, the same behavior of \texttt{Gurobi} can be detected. It starts with reasonable performance but breaks down between 240 and 480 customers, similar to the behavior observed on the large data set.

The \texttt{Decomp} solvers exhibit similar good performance judging by the \coo\ reduction. Interestingly, the per-customer metrics, and therefore also the dominating factor in the energy, measure at a very constant level between the problem sizes. It is once more apparent that \texttt{Gurobi} as a sub-solver outperforms the QUBO-based sub-solvers. Curiously, SA as sub-solver only performs slightly worse than \texttt{Gurobi} in bringing the consumption deviations per customer to a low level but performs almost equally bad in producing few discount changes, similar to the QPU. \texttt{Leap} exhibits similar performance as in our previous experiments. Most notably, although, is that \texttt{Decomp-QPU} seems to perform slightly better than \texttt{Leap} in regard to the optimization objective (much better in regard to the \coo\ reduction). That means that our developed hybrid quantum routine does seem to outperform the general-purpose \texttt{Leap}.
